Green Resilience of Cyber-Physical Systems: Doctoral Dissertation

Cyber-physical systems (CPS) combine computational and physical components. Online Collaborative AI System (OL-CAIS) is a type of CPS that learn online in collaboration with humans to achieve a common goal, which makes it vulnerable to disruptive events that degrade performance. Decision-makers must therefore restore performance while limiting energy impact, creating a trade-off between resilience and greenness. This research addresses how to balance these two properties in OL-CAIS. It aims to model resilience for automatic state detection, develop agent-based policies that optimize the greenness-resilience trade-off, and understand catastrophic forgetting to maintain performance consistency. We model OL-CAIS behavior through three operational states: steady, disruptive, and final. To support recovery during disruptions, we introduce the GResilience framework, which provides recovery strategies through multi-objective optimization (one-agent), game-theoretic decision-making (two-agent), and reinforcement learning (RL-agent). We also design a measurement framework to quantify resilience and greenness. Empirical evaluation uses real and simulated experiments with a collaborative robot learning object classification from human demonstrations. Results show that the resilience model captures performance transitions during disruptions, and that GResilience policies improve green recovery by shortening recovery time, stabilizing performance, and reducing human dependency. RL-agent policies achieve the strongest results, although with a marginal increase in CO2 emissions. We also observe catastrophic forgetting after repeated disruptions, while our policies help maintain steadiness. A comparison with containerized execution shows that containerization cuts CO2 emissions by half. Overall, this research provides models, metrics, and policies that ensure the green recovery of OL-CAIS.

==> Chapters/conference.tex <==
In addition to the three conferences, we stated in the study plan at the begging of this PhD (i) ICSE and (ii) CAIN for the second year, and (iii) ICCPS for the third year, we have published in ISSRE2022 Doctoral Symposium in Charlotte, North Carolina, USA, an \textit{A} ranked conference based on the core conference portal\footnote{International Symposium on Software Reliability Engineering CORE link: \url{http://portal.core.edu.au/conf-ranks/1411/}}, co-chaired by Zheng Zheng, Beihang University, China and Hadi Hemmati, University of Calgary, Canada.


==> Chapters/cooperation.tex <==
This PhD research expects to join \textit{System Srl}\footnote{System Srl link: \url{https://www.system.it/}} between June 2023 - Dec 2023 to study the latest projects in CPS, and possible application of our theories. Additionally, we extend our thanks to \textit{Fraunhofer Italia}, who grant us access to CORAL (Section~\ref{sec:coral}) at Arena labs in NOI TechPark, Bolzano, Italy.

==> Chapters/prelimentary.tex <==
In our preliminary studies, we first conducted a \textbf{systematic literature review (SLR)} to address the research gaps in the field, the review has adopted software engineering guidelines for reporting secondary studies (SEGRESS2022) \cite{kitchenham_segress_2022}. SEGRESS is the \textbf{latest} guideline that defines a systematic process to report literature reviews in software engineering.
The SLR started with more than 560 studies and included more than 175 primary studies,  Figure~\ref{fig:slr} shows the full process of including the studies in the SLR based on SEGRESS guidelines. The main findings are as follows:

\begin{figure}[b]
\centering
\includegraphics[width=.60\textwidth]{Chapters/attach/papersNumberSearchStrategy.pdf}
\caption{Systematic Literature Review Process}
\label{fig:slr}
\index{figures}
\end{figure}

\begin{enumerate}
    \item \textit{Do NOT Just Detect Go for Recovery}: The SLR shows that a small number of studies are actually working on fully recovering the CPS and restoring it to its original state. The SLR shows that only 14 out of 59 studies that handle resilience are fully recovering the CPS, while the rest are stopping on detecting and mitigating the problem to reach an acceptable state. The same applies to studies that handle performance and security issues, \textit{the two main causes of performance degradation}. With 12 studies out of 61 for performance and 14 out of 79 for security. 
    \item \textit{Green, Resilience, and Smart}: Six main learning-based methods have appeared in primary studies included in the SLR, \textit{Deep Learning /Neural Networks}, \textit{Reinforcement Learning}, \textit{Classification Algorithms}, \textit{Linear Regression}, \textit{Semisupervised Learning}, and \textit{Unsupervised Learning}. The SLR shows that the researchers' interest is in using Deep Learning as their solution method to solve fields of research (Green, Energy Consumption, Performance, Security, and Resilience).
    This shows that there is still a research gap in using other learning-based solutions, e.g. the usage of reinforcement learning, which adds a huge contribution especially when mixing it with deep learning \cite{veith_adversarial_2020}, since it allows the system to self-monitor and influence its future behavior \cite{moghadam_autonomous_2022}. Additionally, comparative studies on the usage of these methods can help in creating a systematic approach to optimize resilience and green in CPS.
    \item \textit{CPS Domains}: CPSs are used in various domains like \textit{Smart Grid}, \textit{Industrial CPS}, \textit{Autonomous Driving}, \textit{Health Sector}, \textit{Human with CPS}, and \textit{Robots}. The result of our SLR shows that the robotics, health sectors, and human with CPS fields require more attention due to the lack of research about resilience and green in these systems, and the critical part they play in our nowadays life.
    \item \textit{Novel Approaches}: Solving the trade-off between resilience and green does not stop with smart approaches, the SLR supports exploring different technologies other than learning-based methods to address the trade-off between green and resilience. The problem can be seen as an optimization problem, a game theory problem, or others.
\end{enumerate}

Secondly, we proposed a \textbf{game theory solution} to trade-off between green and resilience. The idea of using game theory is motivated by a tutorial of \textit{Dr. Svetlana Abramova} at the International School on Software Engineering 2022 in Bolzano, Italy \cite{noauthor_ise_nodate}. Game theory is ``the study of rational decision-making between players who seek the best payoffs for their own interest" \cite{mei_engineering_2017}.
The game players, player resilience ($p_1$) and player green ($p_2$) are taking decisions to maximize their own preferences or in other words their \text{utility functions} \cite{von_neumann_theory_2007}.

The game played by $p_1$ and $p_2$ is similar to the \textit{Battle of Sexes} a coordination game between two players that also has the elements of conflict, and each player's decision affects the other \cite{luce_games_1989}. This proposal introduces a new game named \textit{The Gresilience Game}, in this game, the human and robot arm both have a common goal to classify a set of objects based on their color, and they are collaborating in an online learning environment, where the human teaches the robot how to classify the objects. However, during the learning process, the robot will automatically classify objects, that it already learned, but in case of uncertainty, the robot faces some challenges in reaching a high \textit{confidence level} ($\epsilon$ hereinafter, where $\epsilon \in [0, 1]$) of classification about the object's color and deciding whether it should leave the classification to the human, or react and recover. The system in this situation is facing a dilemma because it wants to maintain its performance and move the arm to classify the object, which maximizes the system's resilience. However, if it does and makes a mistake this means wasting more time as the human needs to validate and correct that movement, and also more \coo{} footprint from the extra energy of the wrong movement.


Additional \textbf{academic courses and tutorials} have been done, motivated by the PhD title and the need for a deep understanding of the different innovative technologies. The following are the main courses:

\begin{enumerate}
    \item Cloud Computing and Distributed Systems, at Free University of Bozen-Bolzano. (Motivates the idea of On-Demand learning, Figure~\ref{fig:ondemand}).
    % \item 8$^{th}$ International School on Software Engineering, at Free University of Bozen-Bolzano. (Motivates the idea of Game Theory Solution, Paper~\ref{papers:paperADoctoral}).
    \item Online course about Intro to Cyber-Physical Systems Security Course, at Georgia Institute of Technology\footnote{Course link: \url{https://omscs.gatech.edu/cs-6263-intro-cyber-physical-systems-security-course-videos}}. (Motivates searching for security as a cause of performance degradation in our systematic literature review).
\end{enumerate}


==> Chapters/progresstable.tex <==
\begin{table}[ht!]
\centering
\caption{Thesis progress tracking table}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{Ch/Sec} & \textbf{DR Draft} & \textbf{BR Review} & \textbf{DR R1} & \textbf{AL Review} & \textbf{DR R2} & \textbf{Done?} \\
\hline
Ch.~\ref{ch:intro} & Done &  Done & Done & Done & & \\
Ch.~\ref{ch:background} & Done & Done & Done & & & \\
Ch.~\ref{ch:lr} & Done &Done & & & & \\
Ch.~\ref{ch:methods} & Done & Done& & & & \\
Ch.~\ref{ch:dmframeworks} & Done & Partally & & & & \\
Ch.~\ref{ch:greenresiliencecps} & Done & & & & & \\
Ch.~\ref{ch:coral} & Done & & & & & \\
Ch.\ref{ch:expdesign} & Done & & & & & \\
% Ch.\ref{ch:expexec} & & & & & & \\
Ch.\ref{ch:results} & & & & & & \\
Ch.10 & & & & & & \\
Ch.11 & & & & & & \\
Ch.12 & & & & & & \\
\hline
\end{tabular}
\end{table}


==> Chapters/rqandob.tex <==
This chapter presents the existing research challenges that motivated this PhD research, and the research goals and questions to be addressed.

\section{Research Challenges}
\label{sec:reseachchallenges}
To understand the existing challenges cyber-physical systems (CPS) are facing that motivate this PhD research, we need to set a clear definition of CPS. \textcite{pagliari_case_2017} define CPSs as engineered systems that integrate between the computational algorithms and their physical components, which \textcite{bennaceur_modelling_2019} confirm. Moreover, other studies have pointed out that CPSs are not only the integration between the software parts and the hardware parts of the system but also the communication network between them \cite{barbeau_metrics_2020}.

This work builds on these definitions by stating that CPSs are employed to provide complex \textit{real-time} services by controlling the system physical actuators through the system computational algorithms based on the monitored environment input.

CPS operates in an unpredicted environment, which in many cases does not fully break the CPS and make it not available. But it causes performance degradation, which is no an option for CPS due to the real-time nature of its services. Thus these systems need to have the ability to detect, mitigate and recover to their original state from any performance degradation. This non-functional property is called resilience.

This PhD research is motivated by the following existing research challenges:

\textbf{Building Resilient CPS}: The word resilience has many definitions based on the field it is used in, like psychology, psychiatry, computer science, and other fields \cite{kouicem_artificial_2019}. This proposal focuses on resilience for CPS. Some studies try to define resilience as the maintenance of an acceptable functionality during adverse events \cite{murino_resilience_2019}. While \textcite{haque_contract-based_2018} define it as the fast ability to detect and recover from performance faults,
another definition described resilience as the system's ability to stand against extreme disasters and return to normal operation \cite{ti_resilience_2022}.

\textcite{mouelhi_predictive_2019} have described two properties of CPS resilience, \textit{internal autogenous resilience} that refers to the system's ability to detect and process faults and attacks, and \textit{external resilience}, which is the maintenance of a safe operation within the system surrounding environment.

This PhD research refers to resilience as the ability of the system to detect performance degradation and perform one or more actions to mitigate the degradation and restore it to the original state in the fastest time possible.
Additionally, many studies show a tight relation between resilience and performance degradation, and between resilience and security breaches.

This non-functional property is critical for CPS to continue delivering real-time services. However, this is not an easy task to perform and many studies have proposed various ways to solve the issue, but the research is still open for innovative studies (studies that uses learning-based methods, or cloud computing functionalities, etc.). Moreover, a lot of these studies are discussing how to identify the performance degradation root cause or how to detect a security attack, but only few of them discussing how to fully recover from this anomaly and restore the CPS to its original state.

Furthermore, solutions that build resilience in CPS require additional energy and thus additional \coo{} footprint. This raises an additional challenges when trying to build resilience in CPS, the CPS becomes less environmental-friendly, or in other words, not green, whih leads us to the second research challenge.

\textbf{Maintaining a Green State}: The adopted definition of Green is the definitions of information technological systems (IT-systems) that is \textit{the efficient usage of energy with minimizing adverse effects} \cite{kharchenko_concepts_2017}.
IT-systems are systems responsible for storing, displaying, transforming, and transferring information \cite{kharchenko_concepts_2017}, and CPS is one of these systems.

\coo{} footprint is one of the known direct and indirect adverse from CPS, during development and application \cite{kharchenko_concepts_2017}.
Thus, the challenge is in building a resilient CPS does not require additional energy consumption or computational power.

\section{Research Goals}
% CodeCarbon \cite{mila_codecarbonio_nodate} is a Python lightweight package that estimates the \coo{} footprint coming from cloud/personal computing resources. It can wrap the overall computation code and gives the estimation based on the geographical location of the system under testing.
\label{sec:researchgoals}

This PhD research is promoting green system recovery after unexpected performance degradation (due to some security breaches or performance anomalies) for building resilient CPS through employing innovative software technologies like learning-based techniques, and cloud computing functionalities, to mention a few.

In order to address the aforementioned research challenges, the following research goals are shaping this PhD research. From these goals we derived the following research questions based on Goal Question Matrix Approach (GQM) by \textcite{caldiera_goal_1994}:

\begin{itemize}
    \item \textbf{RG1}: Understand the relation between Green and Resilience in a cyber-physical system context.
    \begin{itemize}
        \item RQ1.1: Are \textit{Green} and \textit{Resilience} adversaries?
        \item RQ1.2: What are the characteristics of the relation between \textit{Green} and \textit{Resilience}?
    \end{itemize}
    \item \textbf{RG2}: Understand how can innovative technologies (machine learning, cloud computing, etc.) be used to build Resilient cyber-physical systems in a Green manner.
    \begin{itemize}
        \item RQ2.1: What are the different causes for \textit{performance degradation} in CPS?
        \item RQ2.2: What are the learning-based methods to detect and recover the degrading in the CPS performance?
        \begin{itemize}
            \item RQ2.2.1: To what extent \textit{Green} is affected by the usage of these methods?
            \item RQ2.2.2: Can the usage of cloud functionalities help to enhance these methods \textit{Green}?
        \end{itemize}
    \end{itemize}
    \item \textbf{RG3}: Discuss the different approaches to trade-off between Green and Resilience in the context of CPS and define their properties and limitations.
    \begin{itemize}
        \item RQ3.1: What is an effective way to achieve \textit{Green} and \textit{Resilience}?
        \begin{itemize}
            \item RQ3.1.1: Does this way has complexity or cost limitations?
        \end{itemize}
        \item RQ3.2: Can the proposed approach to the trade-off between \textit{Green} and \textit{Resilience} be leveraged to other non-functional properties?
    \end{itemize}
    % \item Apply the trade-off approaches to real-life case studies like collaborative artificial intelligence systems, and industrial cyber-physical systems to check whether these approaches can be generalized for all cyber-physical system types.
\end{itemize}

By addressing these goals, we will be able to create an efficient automated approach for cyber-physical systems that solves the green resilience trade-off problem. Moreover, this approach might motivate more studies about how we can trade-off between two other non-functional properties that have a similar relation like green and resilience in the system, and this is another generalization aspect to consider.


% Achieving these objectives requires first, understanding the current state of the art and the research gaps, second, finding a real-life case study, third, understanding what are the possible causes of performance degradation in the system, four, exploring the different methods and actions to recover from this degradation, five, finding the way to each method recovery time and green effect, and six, apply the overall approach on the real-life case study and check whether the applied approach has successfully built a resilient CPS which is green as well, or not.





==> Chapters/rqanswers.tex <==
In this chapter, we address the research questions introduced at the beginning of this PhD thesis. These questions have been systematically organized under three overarching research goals:
\textbf{RG1}: Model the resilience of OL-CAIS behavior to support the decision-makers, \textbf{RG2}: Develop intelligent policies to balance resilience and greenness in OL-CAIS upon unforeseen disruptive events, and \textbf{RG3}: Understand catastrophic forgetting in OL-CAIS in the aftermath of a disruptive event and its resolution.
Each research goal and its associated research questions are presented in the following sections, along with their respective answers derived from the findings of this research.
 
\section{Research Questions Associated to the First Research Goal}
This section addresses \textbf{RG1}, which aims to model the resilience of OL-CAIS behavior to support decision-makers, specifically tackling \textbf{RC1}: Detecting performance degradation. To address this challenge, we conducted evaluations that analyze how OL-CAIS identifies and characterizes disruptive events and their impact on system performance. 
The experiments investigated the evolution of performance across steady, disruptive, and final states, providing insights into how the system transitions between these states and highlighting key metrics such as Average Classification Rate (ACR) and ACR Threshold. 
These evaluations directly contribute to answering the associated research questions by defining performance metrics (RQ1.1), distinguishing acceptable and unacceptable performance levels (RQ1.2), and identifying the states and transitions that reflect resilience (RQ1.3).








\section{Research Questions Associated to the Second Research Goal}
This section focuses on \textbf{RG2}, which aims to develop intelligent policies to balance resilience and greenness in OL-CAIS during unforeseen disruptive events, addressing \textbf{RC2}: Balancing greenness and resilience upon disruptive events. 
Our evaluations investigated various decision-making policies, including internal, one-agent, two-agent, and RL-agent, to understand their impact on system recovery and energy efficiency. 
These experiments, conducted in both real-world and simulated settings, explored the trade-offs between greenness and resilience. 
Additionally, we evaluated the role of containerization as a green resource allocation technology. 
These evaluations contribute to understanding the relationship between greenness and resilience (RQ2.1), the necessary decision-making components (RQ2.2), and the effectiveness of different policies (RQ2.3, RQ2.4). Finally, the containerization experiments directly address how resource optimization enhances energy efficiency (RQ2.5).

\paragraph{Answer to RQ2.1.} \textit{What are the different metrics required to measure resilience and greenness in OL-CAIS?}

OL-CAIS performs one or more actions to complete a specific task. 
The operator of these actions in OL-CAIS varies between the human and the autonomous components. Thus, these actions are either human actions or autonomous actions.
To understand if these actions are resilient or green, it is important to define some metrics that help us measure these attributes or qualities.
We define the action \textit{run time} as a metric to measure resilience and both \textit{CO$_2$ emission} and \textit{number of human interactions} as metrics to measure greenness.
At each iteration in the disruptive state, we can estimate these metrics for the feasible actions by using exponential smoothing, which incorporates their historical values. 

\paragraph{Answer to RQ2.2.} \textit{What are the necessary components to automatically monitor OL-CAIS behavior, and support decision-making?}

We address this research question by defining a decision-making assistant that continuously monitors the evolution of the OL-CAIS performance, detects performance degradation, invokes internal or external decision-making policies, recommends recovery action, and actuates it.
The assistant consists of three components: A \textit{monitoring component} that gives the decision-makers of OL-CAIS a preview of the performance evolution and allows them to select the decision-making policies.
An \textit{actuator component} that connects to the OL-CAIS classifier and tracks the ACR values to identify the system's state.
The actuator invokes the selected decision-making policies to recommend the action to execute and then actuate it on OL-CAIS.
The last component is a \textit{simulator component}, which allows decision-makers to simulate their system's running environment to explore different disrupted events and decision-making policies in a protected environment to facilitate their decisions.
 
\paragraph{Answer to RQ2.3.} \textit{What is the value of different agent policies (one-agent, two-agent, reinforcement-learning-agent) in supporting OL-CAIS to restore its services by balancing greenness and resilience during disruptions?}

\paragraph{Answer to RQ2.3.} \textit{Are the agent-based policies valuable in supporting OL-CAIS to restore its services while balancing greenness and resilience upon disruptions?}

We have conducted various experiments to evaluate the agent-based policies supporting decision-making for green recovery.
We conducted real-world experiments and simulated experiments with two different disruptive events.
From each experiment, we collected the resilience model, the type of action executed, and the CO$_2$ emission.
The results from the real-world experiments show that one-agent policies exhibited a more steady performance than internal policies although our OL-CAIS did not recover. It has reduced the human interactions from both internal and two-agent policies experiments, which indicates an autonomous attempt to restore performance. 
The two-agent policies show intermediate results between one-agent and RL-agent. RL-agent shows superior results compared to one-agent and two-agent in terms of rapid recovery and higher autonomous ratio. However, it comes at a higher CO$_2$ emission cost as it requires more computational power than the other agent-based policies. 
The simulated results generalize these findings.
The change in the disruptive event did not have much effect on the overall findings. We just noticed that some disruptive events with less disruption effect lead to faster recovery.

\paragraph{Answer to RQ2.4.} \textit{What are the major differences between the agent policies in terms of resilience and greenness?}

To address this research question, we have defined a measurement framework that addresses resilience and greenness qualities through two concepts each: recovery speed and performance steadiness indicate the effectiveness of decision-making policies toward resilience, while green efficiency and autonomy indicate the effectiveness of decision-making policies toward greenness.
We define the duration ratio of the recovering state as a metric to measure recovery speed, the performance fluctuation metric measures performance steadiness, the CO$_2$ emission mean metric measures green efficiency, and the human-dependency metric measures autonomy. Minimizing each of these metrics indicates a higher level of greenness and resilience.

Fig.~\ref{fig:darknesssimureal} shows the measurement framework metrics. The column in the chart represents the average of these metrics in the one hundred experiments of each decision-making policies. While the black dot is the data coming from real-world experiments. We aggregate both results using the same disruptive event in these experiments (i.e., turn off the lights and the darkness filter).
We notice that some of these dots are far from the one hundred experiment average. However, these dots are still within the bounds of the data. For example, the duration ratio of the recovering state in the real-world experiment was 0.96, as the system had never recovered.
However, the upper bound of the one-agent's duration ratio of the recovering state was $1.29$, and since $0.96 < 1.29$, this experiment does not represent an outlier.

\begin{figure}[ht!]
\centering
\centerline{\includegraphics[width = \textwidth]{Chapters/attach/part3/darkness_simu_real.pdf}}
\caption{Measurement framework results from simulated and real-world experiments with darkness disruptive event.}
\label{fig:darknesssimureal}
\end{figure}

TODO here, put the experiment from histogram equalizer.

\paragraph{Answer to RQ2.5.} \textit{How can we optimize resource allocation using containerization to ensure efficient energy consumption?}

We have defined a new methodology to wrap the multi-machinery bare-metal setup with containers in our attempt to save energy consumption. By applying our methodology to our collaborative robot CORAL, we have reduced the energy consumption and thus its adverse effect (i.e., CO$_2$ emission) to half the bare-metal setup. 
Furthermore, by wrapping the OL-CAIS components in docker containers, we were able to use docker-compose to orchestrate these containers, creating replicas of the components, which increased our system resilience toward component failure and reduced the response time as everything was running on a localhost network.

\section{Research Questions Associated to the Third Research Goal}
This section addresses \textbf{RG3}, which aims to understand catastrophic forgetting in OL-CAIS following disruptive events and their resolution, tackling \textbf{RC3}: Understanding catastrophic forgetting. 
Our evaluations examined whether the system retains memory of steady-state settings after resolving disruptions, highlighting the potential for catastrophic forgetting. 
These evaluations also investigated mitigation strategies, such as using intelligent policies, to maintain consistent performance over time. 
These experiments analyze patterns in resilience models and assess transitions between steady, disruptive, and final states. They provide evidence for detecting catastrophic forgetting (RQ3.1) and suggest strategies to ensure steady performance (RQ3.2).

\paragraph{Answer to RQ3.1.} \textit{What are the patterns in the resilience model that indicate catastrophic forgetting in OL-CAIS?}

In all our real-world or simulated experiments, we have noticed that the OL-CAIS classifier maintains a memory from the disruptive state. This means when we fixed the disruptive event and restored the original environment settings as they were in the steady state, the classifier forgot the original environment and experienced a second performance degradation. 
In the final state, we observed that the system started learning again from human interactions as this was the first time to see these objects. 
Thus, a second performance degradation state is a clear indication of catastrophic forgetting in OL-CAIS going out from a disruptive state.

\paragraph{Answer to RQ3.2.} \textit{How can we ensure that OL-CAIS maintains steady performance over time, even when facing frequent disruptions?}

Our current solution considers the fixed event another disruptive event. In other words, any performance degradation is a cause of some disruptive event.
Thus, we always put the system under the GResilience decision-making policies to ensure consistent, steady performance and fast recovery.



==> Chapters/wishlist.tex <==
Future work:

A state machine consists of several machine learning models and a main model that determines whether a state is an anomaly state, a new state, or one of the existing states.
Then, this leading model moderates between these states without affecting the learning rate of the different machine learning models.


?? what if the threshold in the stready state was zero (the minimum)?



Finally, for a comprehensive OL-CAIS that considers greenness and resilience, not only in design but in run-time, we aim to integrate our decision-making toolbox as an intermediate container that monitors the interaction between the system containers and redirects the decisions to ensure a balance between greenness and resilience. This will be further discussed in future work.



==> Chapters/workplan.tex <==
The main milestones of this PhD research are:

\begin{enumerate}[label=M\arabic*.]
    \item PhD Study Plan.
    \item Systematic Literature Review.
    \item Working with CORAL (see Section~\ref{sec:coral}).
    \item Propose Solution to Achieve the Research Goals.
    \item Working with System Srl.
    \item Understand Possible Case Studies and Data Collection.
    \item Conducting Empirical Studies.
    \item Validation.
    \item Thesis Writing.
\end{enumerate}
\newpage
Figure~\ref{fig:timetable} shows a tabular representation of the expected schedule of these milestones during the PhD study time frame.

\begin{figure}[hbt!]
\centering
\includegraphics[width=\textwidth]{Chapters/attach/Timetable.pdf}
\caption{PhD Timeline}
\label{fig:timetable}
\index{figures}
\end{figure}

% M1 – Preliminary work
% M2 – Development of a framework
% M3 – Define variables and Develop measuring Tools
% M4 – Selection of appropriate Machine learningAI Models
% M5 – Data Collection, training, and testing models
% M6 – Analysis, and  interpretation of results
% M7 – Validation
% M8 – Thesis writing

